Deterministic Decremental SSSP and Approximate Min-Cost Flow in Almost-Linear Time

In the decremental single-source shortest paths problem, the goal is to maintain distances from a fixed source $s$ to every vertex $v$ in an $m$-edge graph undergoing edge deletions. In this paper, we conclude a long line of research on this problem by showing a near-optimal deterministic data structure that maintains $(1+\epsilon)$-approximate distance estimates and runs in $m^{1+o(1)}$ total update time. Our result, in particular, removes the oblivious adversary assumption required by the previous breakthrough result by Henzinger et al. [FOCS'14], which leads to our second result: the first almost-linear time algorithm for $(1-\epsilon)$-approximate min-cost flow in undirected graphs where capacities and costs can be taken over edges and vertices. Previously, algorithms for max flow with vertex capacities, or min-cost flow with any capacities required super-linear time. Our result essentially completes the picture for approximate flow in undirected graphs. The key technique of the first result is a novel framework that allows us to treat low-diameter graphs like expanders. This allows us to harness expander properties while bypassing shortcomings of expander decomposition, which almost all previous expander-based algorithms needed to deal with. For the second result, we break the notorious flow-decomposition barrier from the multiplicative-weight-update framework using randomization.

==> max_macros_temp.tex <==
\global\long\def\dist{\mathbf{dist}}
\global\long\def\distEst{\tilde{d}}
\global\long\def\shortestSTPathVar{\pi(s,t)}

\global\long\def\flowVar{f}
\global\long\def\flowEstVar{\hat{f}}
\global\long\def\costEstVar{\hat{c}}
\global\long\def\initialDifferenceMWU{\delta}
\global\long\def\flowRouted{\Upsilon}

\global\long\def\weightFunctionVar{w}
\global\long\def\weightFunctionEstVar{\Hat{w}}
\global\long\def\weightFunctionCombinedVar{\tilde{w}}

\global\long\def\costFunctionVar{\varphi}
\global\long\def\costFunctionEstVar{\hat{\varphi}}

\global\long\def\inflow{\textrm{in}}
\global\long\def\outflow{\textrm{out}}

\global\long\def\edgeSensitivity{\sigma}
\global\long\def\sensitivity{\sigma}

\global\long\def\neighborhood{\mathcal{N}}

\global\long\def\objFunctionVar{\textsc{ObjVal}}
\global\long\def\objFunctionEstVar{\widehat{\textsc{ObjVal}}}

\global\long\def\timeAugSSSPVar{\mathcal{T}_{SSSP^{\pi}}

\global\long\def\minCapIndexMWUVar{\Lambda}
\global\long\def\forLoopIndexMWU{\lambda}

\newcommand{\shortestSTPath}[1][]{
	\ifthenelse{\equal{#1}{}}{\shortestSTPathVar}{\shortestSTPathVar_{#1}}
}

\newcommand{\costFunction}[1][]{
	\ifthenelse{\equal{#1}{}}{\costFunctionVar}{\costFunctionVar_{#1}}
}

\newcommand{\costFunctionEst}[1][]{
	\ifthenelse{\equal{#1}{}}{\costFunctionEstVar}{\costFunctionEstVar_{#1}}
}

\newcommand{\weightFunction}[1][]{
	\ifthenelse{\equal{#1}{}}{\weightFunctionVar}{\weightFunctionVar_{#1}}
}

\newcommand{\weightFunctionEst}[1][]{
	\ifthenelse{\equal{#1}{}}{\weightFunctionEstVar}{\weightFunctionEstVar_{#1}}
}

\newcommand{\weightFunctionCombined}[1][]{
	\ifthenelse{\equal{#1}{}}{\weightFunctionCombinedVar}{\weightFunctionCombinedVar_{#1}}
}

\newcommand{\flow}[1][]{
	\ifthenelse{\equal{#1}{}}{\flowVar}{\flowVar_{#1}}
}

\newcommand{\flowEst}[1][]{
	\ifthenelse{\equal{#1}{}}{\flowEstVar}{\flowEstVar_{#1}}
}

\newcommand{\costEst}[1][]{
	\ifthenelse{\equal{#1}{}}{\costEstVar}{\flowEstVar_{#1}}
}

\newcommand{\minCapIndexMWU}[1][]{
	\ifthenelse{\equal{#1}{}}{\minCapIndexMWUVar}{\minCapIndexMWUVar_{#1}}
}

\newcommand{\objFunction}[1][]{
	\ifthenelse{\equal{#1}{}}{\objFunctionVar}{\objFunctionVar_{#1}}
}

\newcommand{\objFunctionEst}[1][]{
	\ifthenelse{\equal{#1}{}}{\objFunctionEstVar}{\objFunctionEstVar_{#1}}
}

\newcommand{\timeAugSSSP}[7]{
	\timeAugSSSPVar(#1, #2, #3, #4, #5, #6,#7)
}



==> together_distance.tex <==

\section{Putting Distance-only Components Together}

In this section, we show how all our data structures fit together.
The main data structures were $\Apxball$(\ref{def:Apxball}), $\Core$(\ref{def:Core}),
and Covering(\ref{def:Covering}).
\begin{theorem}
\label{thm:main no distance}For any $n$ and $\eps\in(\phicmg,0.1)$,
let $G=(V,E)$ be a decremental bounded-degree graph with $n$ vertices
and edge weights are from $\{1,2,\dots,W=n^{2}/\eps\}$. Let $S\subseteq V$
be any decremental set. We can implement $\Apxball(G,S,\eps)$ using
$\Ohat(n)$ total update time.
\end{theorem}

There are \emph{distance scales} $D_{0}\le D_{1}\le\dots\le D_{\distScale}$
where $D_{i}=(nW)^{i/\distScale}$ and $\distScale=c_{\distScale}\lg\lg\lg n$
for some small constant $c_{\distScale}>0$. We will implement our
data structures for $\distScale$ many levels. Recall that $\phicmg=1/2^{\Theta(\log\log n)^{2}}=\Omegahat(1)$
from \ref{sec:prelim}. For $0\le i\le\distScale$, we set 
\begin{align*}
k_{i} & =(\lg\lg n)^{3^{i}}\\
\gamma_{i} & =1/\phicmg^{6k_{i+1}}\text{ and }\gamma_{-1}=1\\
\eps_{i} & =\eps/50^{\distScale-i}\\
\stretch_{i} & =\gamma_{i-1}\cdot\log^{c_{\stretch}}n/\phicmg^{3}\\
\Delta_{i} & =\Theta(k_{i}n^{2/k_{i}}/\phicmg)
\end{align*}
where we define $c_{\stretch}$ to be a large enough constant. The parameters
are defined in such that way that 
\[
n^{1/\distScale},\frac{D_{i}}{D_{i-1}},n^{1/k_{i}},\gamma_{i},1/\eps_{i},\stretch_{i},\Delta_{i}=\Ohat(1)
\]
 for all $0\le i\le\distScale$. (By contrast, note that $D_{i}$
ranges from $1$ to $nW=\poly(n)$.) To exploit these parameters,
we need more fine-grained properties which are summarized below:
\begin{prop}
\label{prop:para}For large enough $n$ and for all $0\le i\le\distScale$,
we have that 
\begin{enumerate}
\item \label{enu:para:k}$\lg\lg n\le k_{i}\le(\lg^{1/100}n)$, 
\item $\phicmg^{2}\le\eps_{i}\le\eps$
\item $\gamma_{i}=2^{O((\lg^{1/100}n)(\lg\lg n)^{2})}$, 
\item \label{enu:para:D ratio}$D_{i}/D_{i-1}\le n^{4/\distScale}$,
\item \label{enu:para:gap and distance scale}$\gamma_{i}\le D_{i}/D_{i-1}$,
and
\item \label{enu:para:key}$\gamma_{i}\ge(\gamma_{i-1}\cdot\frac{1}{\phicmg^{6}})^{k_{i}}\ge(\frac{\stretch_{i}}{\eps_{i}})^{k_{i}}$.
\end{enumerate}
\end{prop}

\begin{proof}
(1): We have $k_{i}=(\lg\lg n)^{3^{i}}\le(\lg\lg n)^{3^{\distScale}}\leq(\lg\lg n)^{(\lg\lg n)^{1/100}}\le\lg^{1/100}n$
as $\distScale=c_{\distScale}\lg\lg\lg n$ and $c_{\distScale}$ is
a small enough constant. 

(2): It is clear that $\eps_{i}\le\eps$. For the other direction,
note that in the assumption of \ref{thm:main no distance}, we have
$\eps\ge\phicmg$. So $\eps_{i}\ge\eps/50^{\distScale}\ge\phicmg/50^{\Theta(\lg\lg\lg n)}\ge\phicmg^{2}$
because $\phi=1/2^{\Theta(\lg\lg n)^{2}}$.

(3): As $\frac{1}{\phicmg}=2^{\Theta(\lg\lg n)^{2}}$and $\gamma_{i}=1/\phicmg^{6k_{i+1}}$,
we have from property \ref{enu:para:k} of this proposition that $\gamma_{i}=2^{O((\lg^{1/100}n)(\lg\lg n)^{2})}$. 

(4): We have $D_{i}/D_{i-1}=(nW)^{1/\distScale}$. Since $W=n^{2}/\eps\le n^{3}$, we have $D_{i}/D_{i-1}\le n^{4/\distScale}$.

(5): As $D_{i}/D_{i-1}\ge n^{1/\distScale}\ge2^{\Theta(\lg n/\lg\lg\lg n)}$,
by (2) we have $\gamma_{i}\le(D_{i}/D_{i-1})$ when $n$ is large
enough.

(6): We have $\gamma_{i}\ge(\gamma_{i-1}\cdot\frac{1}{\phicmg^{6}})^{k_{i}}$
because
\[
\gamma_{i}=(\frac{1}{\phicmg^{6}})^{k_{i+1}}\ge(\frac{1}{\phicmg^{6}})^{(k_{i}^{2}+k_{i})}=((\frac{1}{\phicmg^{6}})^{k_{i}}\cdot\frac{1}{\phicmg^{6}})^{k_{i}}=(\gamma_{i-1}\cdot\frac{1}{\phicmg^{6}})^{k_{i}}
\]
where the inequality holds is because $k_{i+1}=(\lg\lg n)^{3^{i+1}}=(\lg\lg n)^{3^{i}\cdot2}\times(\lg\lg n)^{3^{i}}\ge(\lg\lg n)^{3^{i}\cdot2}+(\lg\lg n)^{3^{i}}=k_{i}^{2}+k_{i}$
for all $i\ge0$. For the second inequality, we have 
\[
\frac{\stretch_{i}}{\eps_{i}}=\frac{\gamma_{i-1}(\log^{c_{\stretch}}n)/\phicmg^{3}}{\eps_{i}}\le\frac{\gamma_{i-1}}{\phicmg^{6}}
\]
because $(\log^{c_{\stretch}}n)\le1/\phicmg$ and $\eps_{i}\ge\phicmg^{2}$
by (2). Therefore, $\gamma_{i}\geq(\gamma_{i-1}\cdot\frac{1}{\phicmg^{6}})^{k_{i}}\ge(\frac{\stretch_{i}}{\eps_{i}})^{k_{i}}$.
\end{proof}


\begin{lem}
\label{lem:main induction}For $0\le i\le\distScale$, we can maintain
the following data structures:
\begin{enumerate}
\item \label{enu:induction ball}$\Apxball(G,S,d',\eps_{i})$ for any $d'\le32D_{i+1}\log(n)/\eps_{i}$
using total update time of 
\[
\Otil(\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}})=\Ohat(\left|\ball_{G}(S,d')\right|).
\]
\item $\Core(G,\Kinit,d')$ for any $d'\le D_{i+1}$ using total update
time of 
\[
\left|\ball_{G}(S,32d'\log n)\right|\poly(\frac{n^{1/k_{0}+1/\distScale}}{\phicmg\eps_{0}})=\Ohat(\left|\ball_{G}(S,32d'\log n)\right|)
\]
with scattering parameter $\scatter=\Omega(\phicmg)$ and stretch
at most $\stretch_{i}$.
\item $(D_{i},k_{i},\eps_{i},\stretch_{i},\Delta_{i})$-covering using total
update time of $\Otil(n\cdot\poly(\frac{n^{1/k_{0}+1/\distScale}}{\phicmg\eps_{0}}))=\Ohat(n)$.
\end{enumerate}
For all $i>0$, we assume by induction that a $(D_{i-1},k_{i-1},\eps_{i-1},\stretch_{i-1},\Delta_{i-1})$-covering
is already explicitly maintained.
\end{lem}

\begin{proof}
(1): We prove by induction that the total update time is $\left|\ball_{G}(S,d')\right|\cdot(i+1)\cdot\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}}\cdot(\log n)^{c'}$
where where $c'$ is some large enough constant. For $i=0$, we have
by \ref{prop:ES tree} that
\begin{align*}
\Apxball(G,S,d',\eps_{i}) & \le O(\left|\ball_{G}(S,d')\right|d')\\
 & \le\left|\ball_{G}(S,d')\right|\cdot O(D_{1}\log(n)/\eps_{1})\\
 & \le\left|\ball_{G}(S,d')\right|\cdot(i+1)\cdot\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}}\cdot(\log n)^{c'}.
\end{align*}

For $i>0$, we assume $d'\ge32D_{i}\log(n)/\eps_{i-1}$ otherwise
we are done by induction hypothesis (See \ref{enu:induction ball}
of \ref{lem:main induction}). Note that $D_{i}\ge\gamma_{i}D_{i-1}\ge(\frac{\stretch_{i}}{\eps_{i}})^{k_{i}}D_{i-1}$
by \ref{prop:para}(\ref{enu:para:gap and distance scale} and \ref{enu:para:key}).
So 
\[
d'\ge\frac{32\log n}{\eps_{i-1}}D_{i}\ge\frac{32\log n}{\eps_{i-1}}\cdot(\frac{\stretch_{i}}{\eps_{i}})^{k_{i}}D_{i-1}\ge2(\frac{\stretch_{i-1}}{\eps_{i-1}})^{k_{i-1}}D_{i-1}
\]
where the last inequality is because $k_{i}\ge k_{i-1}$ and $\frac{\stretch_{i}}{\eps_{i}}\ge\frac{\stretch_{i-1}}{\eps_{i-1}}$.
As $(D_{i-1},k_{i-1},\eps_{i-1},\stretch_{i-1},\Delta_{i-1})$-covering
is already explicitly maintained, by \ref{thm:Apxball}, we can maintain
$\Apxball(G,S,d',\eps_{i})$ where $\eps_{i}=50\eps_{i-1}$ using
total update time of 
\begin{align*}
 & \Otil(\left|\ball_{G}(S,d')\right|\Delta_{i-1}\frac{(32D_{i+1}\log(n)/\eps_{i})}{\eps_{i-1}D_{i-1}})+T_{\Apxball}(G,S,2(\frac{\stretch_{i-1}}{\eps_{i-1}})^{k_{i-1}}D_{i-1},\eps_{i-1})\\
 & \le\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{i-1}+8/\distScale}}{\phicmg\eps_{i-1}^{2}}\cdot(\log n)^{c'}+T_{\Apxball}(G,S,d',\eps_{i-1}) & \text{by \ref{prop:para}(\ref{enu:para:D ratio})}\\
 & \le\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}}\cdot(\log n)^{c'}+i\left|\ball_{G}(S,d')\right|\cdot\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}}\cdot(\log n)^{c'} & \text{by IH}\\
 & =(i+1)\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+8/\distScale}}{\phicmg\eps_{0}^{2}}\cdot(\log n)^{c'}.
\end{align*}

(2): For $i=0$, we have that a $(1,1,O(1))$-compressed graph of
$G$ can be trivially maintained by \ref{prop:compressed base}. By
\ref{thm:Core}, we can implement $\Core(G,\Kinit,d')$ with scattering
parameter $\scatter=\Omega(\phicmg)$ and stretch at most $\Otil(1/\phicmg^{3})\le\stretch_{0}$
(by definition of $\stretch_{0}$) with total update time 
\[
\Otil\left(T_{\Apxball}(G,\Kinit,32d'\log n,0.1)(D_{1})^{3}/\phicmg^{2}\right)=\Otil\left(|\ball_{G}(\Kinit,32d'\log n)|D_{1}{}^{4}/\phicmg^{2}\right)
\]
by \ref{prop:ES tree}. 

For $i>0$, given that a $(D_{i-1},k_{i-1},\eps_{i-1},\stretch_{i-1},\Delta_{i-1})$-covering
is explicitly maintained, by \ref{prop:core-compressed is compressed},
we can automatically maintain a $(D_{i-1},\gamma_{i-1},\Delta_{i-1})$-compressed
graph where $\gamma_{i-1}\ge(\stretch_{i-1}/\eps_{i-1})^{k_{i-1}}$
by \ref{prop:para}(\ref{enu:para:key}).\textbf{ }By \ref{thm:Core},
we can maintain $\Core(G,\Kinit,d')$ with $\scatter=\Omega(\phicmg)$
and $\Otil(\gamma_{i-1}/\phicmg^{3})\le\stretch_{i}$ (by definition
of $\stretch_{i}$) with total update time 
\begin{align*}
\Otil\left(T_{\Apxball}(G,\Kinit,32d'\log n,0.1)\Delta_{i-1}^{2}(D_{i+1}/D_{i-1})^{3}/\phicmg^{2}\right) & =\left|\ball_{G}(\Kinit,32d'\log n)\right|\poly(\frac{n^{1/k_{0}+1/\distScale}}{\phicmg\eps_{0}})
\end{align*}
by (1). 

(3): Recall that the algorithm from \ref{thm:covering} for maintaining
a $(D_{i},k_{i},\eps_{i},\stretch_{i},\Delta_{i})$-covering of $G$
assumes, for all $D_{i}\le d'\le D_{i}(\frac{\stretch_{i}}{\eps_{i}})^{k}$,
$\Core$ and $\Apxball$ data structures with input distance parameter
$d'$. By (1) and (2), we can indeed implement these data structures
for any distance parameter $d'\le D_{i+1}$. Since $D_{i}(\frac{\stretch_{i}}{\eps_{i}})^{k_{i}}\le D_{i}\gamma_{i}\le D_{i+1}$
by \ref{prop:para}(\ref{enu:para:key},\ref{enu:para:gap and distance scale}),
the assumption is satisfied. 

So, using \ref{thm:covering}, we can maintain $(D_{i},k_{i},\eps_{i},\stretch_{i},\Delta_{i})$-covering
of $G$ with $\Delta_{i}=\Theta(k_{i}n^{2/k_{i}}/\scatter)$ in total
update time of 
\[
O(k_{i}n^{1+2/k_{i}}\log n/\scatter+\sum_{C\in\cC^{ALL}}T_{\Core}(\stage G{t_{C}},\stage C{t_{C}},d_{\Clevel(C)})+T_{\Apxball}(\stage G{t_{C}},\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i}}32d,\eps_{i}))
\]
where $\cC^{ALL}$ contains all cores that have ever been initialized
and, for each $C\in\cC^{ALL}$, $t_{C}$ is the time $C$ is initialized.
By plugging in the total update time of $\Apxball$ from (1) and $\Core$
from (2), the total update time for maintaining the covering is 
\[
\Otil(\frac{n^{1+2/k_{i}}}{\scatter}+\sum_{C\in\cC^{ALL}}\left|\ball_{\stage G{t_{C}}}(\stage C{t_{C}},32d_{\Clevel(C)}\log n)\right|\poly(\frac{n^{1/k_{0}+1/\distScale}}{\phicmg\eps_{0}})+\left|\ball_{\stage G{t_{C}}}(\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i}}d_{\Clevel(C)})\right|\frac{n^{2/k_{0}+4/\distScale}}{\phicmg\eps_{0}^{2}}).
\]
As it is guaranteed by \ref{thm:covering} that $\sum_{C\in\cC^{ALL}}|\ball_{\stage G{t_{C}}}(\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i}}d_{\Clevel(C)})|\le O(k_{i}n^{1+2/k_{i}}/\scatter)$,
the above expression simplifies to $\Otil(n\cdot\poly(\frac{n^{1/k_{0}+1/\distScale}}{\phicmg\eps_{0}}))$.
\end{proof}
By constructing all the data structures from level $i=0$ to $\distScale$,
we can conclude \ref{thm:main no distance}.

\begin{figure}
\includegraphics[width=0.8\textwidth]{scheme}

\caption{Overall scheme}
\end{figure}



==> together_path.tex <==

\section{Putting Path-reporting Components Together}

\label{sec:together_path}

In this section, we show how to recursively combine all path-reporting
data structures including $\Apxball^{\pi}$(\Cref{def:Apxball path}),
$\Core^{\pi}$ (\Cref{def:Core path}), and path-reporting Covering  (\Cref{def:Covering path})
to obtain the desired decremental path-reporting $\SSSP^{\pi}$ data
structure. The goal of this section is to prove the following theorem.
\begin{theorem}
\label{thm:main path}For any $n$ and $\eps\in(\phicmg,1/500)$,
let $G=(V,E)$ be a decremental bounded-degree graph with $n$ vertices,
edge weights from $\{1,2,\dots,W=n^{5}\}$, and edge steadiness from
$\{0,\dots,\sigma_{\max}\}$ where $\sigma_{\max}=o(\log^{3/4}n)$.
Let $S\subseteq V$ be any decremental set. We can implement $\Apxball^{\pi}(G,S,\eps,\Ohat(1))$
that has $\Ohat(n)$ total update time and query-time overhead of
$(O(\log^{2}n),\Ohat(1))$.
\end{theorem}

As $\SSSP^{\pi}$ is a special case of $\Apxball^{\pi}$ when the
source set $S=\{s\}$, by applying the reduction from \Cref{prop:simplify path},
we immediately obtain \Cref{thm:main SSSP path}, the main result of
this part of the paper. It remains to prove \Cref{thm:main path}.

Define $G_{j}=\sigma_{\ge j}(G)$ for each $j\in\{0,\dots,\sigma_{\max}\}$.
Note that $G_{0}=G$ and $G_{\sigma_{\max}+1}=\emptyset$. There are
\emph{distance scales} $D_{0}\le D_{1}\le\dots\le D_{\distScale}$
where $D_{i}=(nW)^{i/\distScale}$ and $\distScale=c_{\distScale}\lg\lg\lg n$
for some small constant $c_{\distScale}>0$. We will implement our
data structures for $\distScale$ many levels. Recall that $\phicmg=1/2^{\Theta(\log^{3/4}n)}=\Omegahat(1)$
and $\lenapsp=2^{\Theta(\log^{7/8}n)}=\Ohat(1)$. For $0\le i\le\distScale$
and $0\le j\le\sigma_{\max}$, we set 
\begin{align*}
k_{i} & =(\lg\lg n)^{3^{i}}\\
\gamma_{i} & =\lenapsp^{2k_{i+1}}\text{ and }\gamma_{-1}=1\\
\eps_{i,j} & =\eps/(600^{\distScale-i}\cdot2^{j})\text{ and }\eps_{i,\sigma_{\max}+1}=0\\
\stretch_{i} & =\gamma_{i-1}\cdot\lenapsp\log^{c_{\stretch}}n/\phicmg^{2}\\
\Delta_{i} & =\Theta(k_{i}n^{2/k_{i}}/\phicmg)\\
\beta_{i} & =\beta_{i-1}\cdot21\lenapsp\Delta_{i-1}\text{ and }\beta_{0}=7\lenapsp
\end{align*}
where we define $c_{\stretch}$ to be a large enough constant. We
also define parameters related to query-time overhead, for $0\le i\le\distScale$
and $0\le j\le\sigma_{\max}$, as follows:

\begin{align*}
q_{\phi}^{(i,j)} & =c_{q}(\sigma_{\max}-j+1)\log n\\
Q_{\phi}^{(i,j)} & =c_{q}(\sigma_{\max}-j+1)12^{i}\log n\\
\overhead_{\path} & =\frac{n^{2/k_{0}}\lenapsp}{\eps_{0,\sigma_{\max}}^{2}\phicmg^{2}}\log^{c_{q}}(n)\cdot\sigma_{\max}12^{\distScale}\\
q_{\path}^{(i,j)} & =(2i+1)\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}\\
Q_{\path}^{(i,j)} & =2(i+1)\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}
\end{align*}
where $c_{q}$ is a large enough constant. The parameters are defined
in such that way that 
\[
n^{1/\distScale},\frac{D_{i}}{D_{i-1}},n^{1/k_{i}},\gamma_{i},1/\eps_{i,j},\stretch_{i},\Delta_{i},\beta_{i},q_{\phi}^{(i,j)},Q_{\phi}^{(i,j)},q_{\path}^{(i,j)},Q_{\path}^{(i,j)}=\Ohat(1)
\]
for all $0\le i\le\distScale$ and $0\le j\le\sigma_{\max}$. However,
we will need a more fine-grained property of them as described below.
\begin{prop}
\label{prop:para path}For large enough $n$ and for all $0\le i\le\distScale$
and $0\le j\le\sigma_{\max}$, we have that 
\begin{enumerate}
\item \label{enu:para:k path}$\lg\lg n\le k_{i}\le(\lg^{1/100}n)$, 
\item \label{enu:para:eps path}$\phicmg^{2}\le\eps_{i,j}\le\eps$ and $\eps_{i,j}=300\eps_{i-1,j}+\eps_{i,j+1}$,
\item \label{enu:para:gamma path}$\gamma_{i}=2^{O(\lg^{7/8+1/100}n)}$, 
\item \label{enu:para:D ratio path}$D_{i}/D_{i-1}\le n^{6/\distScale}$, 
\item \label{enu:para:gap and distance scale path}$\gamma_{i}\le D_{i}/D_{i-1}$, 
\item \label{enu:para:key path}$\gamma_{i}\ge(\gamma_{i-1}\lenapsp^{2})^{k_{i}}\ge(\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}})^{k_{i}}$,
and
\item \label{enu:para:beta}$\beta_{i}=2^{O((\log^{7/8}n)(\log\log\log n))}\cdot n^{O(1/\lg\lg n)}$.
\end{enumerate}
\end{prop}

\begin{proof}
(1): We have $k_{i}=(\lg\lg n)^{3^{i}}\le(\lg\lg n)^{3^{\distScale}}\leq(\lg\lg n)^{(\lg\lg n)^{1/100}}\le\lg^{1/100}n$
as $\distScale=c_{\distScale}\lg\lg\lg n$ and $c_{\distScale}$ is
a small enough constant.

(2): It is clear that $\eps_{i,j}\le\eps$. For the other direction,
note that in the assumption of \Cref{thm:main no distance}, we have
$\eps\ge\phicmg$. So $\eps_{i}\ge\eps/(600^{\distScale}\cdot2^{\sigma_{\max}})\ge\phicmg/2^{\Theta(\lg\lg\lg n+\sigma_{\max})}\ge\phicmg^{2}$
because $\phicmg=1/2^{\Theta(\lg^{3/4}n)}$ and $\sigma_{\max}=o(\log^{3/4}n)$.
Next, we have $300\eps_{i-1,j}+\eps_{i,j+1}=\eps(\frac{300}{600^{\distScale-(i-1)}\cdot2^{j}}+\frac{1}{600^{\distScale-i}\cdot2^{j+1}})=\eps(\frac{300/600}{600^{\distScale-i}\cdot2^{j}}+\frac{1/2}{600^{\distScale-i}\cdot2^{j}})=\eps(\frac{1}{600^{\distScale-i}\cdot2^{j}})=\eps_{i,j}$.

(3): As $\lenapsp=2^{\Theta(\lg^{7/8}n)}$ and $\gamma_{i}=\lenapsp^{2k_{i+1}}$,
we have from \Cref{enu:para:k} of this proposition that $\gamma_{i}=2^{O(\lg^{7/8+1/100}n)}$.

(4): We have $D_{i}/D_{i-1}=(nW)^{1/\distScale}$. Since $W=n^{5}$,
we have $D_{i}/D_{i-1}\le n^{6/\distScale}$.

(5): As $D_{i}/D_{i-1}\ge n^{1/\distScale}\ge2^{\Theta(\lg n/\lg\lg\lg n)}$,
by \Cref{enu:para:gamma} we have $\gamma_{i}\le(D_{i}/D_{i-1})$ when
$n$ is large enough.

(6): We have $\gamma_{i}\ge(\gamma_{i-1}\lenapsp^{2})^{k_{i}}$ because
\[
\gamma_{i}=\lenapsp^{2}{}^{k_{i+1}}\ge\lenapsp^{2(k_{i}^{2}+k_{i})}=(\lenapsp^{2k_{i}}\cdot\lenapsp^{2})^{k_{i}}=(\gamma_{i-1}\lenapsp^{2})^{k_{i}}
\]
where the inequality holds is because $k_{i+1}=(\lg\lg n)^{3^{i+1}}=(\lg\lg n)^{3^{i}\cdot2}\times(\lg\lg n)^{3^{i}}\ge(\lg\lg n)^{3^{i}\cdot2}+(\lg\lg n)^{3^{i}}=k_{i}^{2}+k_{i}$
for all $i\ge0$. For the second inequality, we have 
\[
\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}}=\frac{\gamma_{i-1}\lenapsp\log^{c_{\stretch}}n/\phicmg^{2}}{\eps_{i,\sigma_{\max}}}\le\frac{\gamma_{i-1}\lenapsp}{\phicmg^{6}}\le\gamma_{i-1}\lenapsp^{2}
\]
because $(\log^{c_{\stretch}}n)\le1/\phicmg$, $\eps_{i,\sigma_{\max}}\ge\phicmg^{2}$
by \Cref{enu:para:eps path}, and $\lenapsp\ge\poly(1/\phicmg)$ when
$n$ is large enough. Therefore, $\gamma_{i}\geq(\gamma_{i-1}\lenapsp^{2})^{k_{i}}\ge(\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}})^{k_{i}}$.

(7): We have $\beta_{i}\le\beta_{\distScale}=\prod_{i=0}^{\distScale}\Otil(\lenapsp n^{2/k_{i}}/\phicmg)=2^{O((\log^{7/8}n)(\log\log\log n))}\prod_{i=0}^{\distScale}n^{2/k_{i}}$
by definition of $\lenapsp,\phicmg$ and $\distScale$. As $\sum_{i=0}^{\dist}1/(\lg\lg n)^{3^{i}}=O(1/\lg\lg n)$,
we have $\prod_{i=0}^{\distScale}n^{2/k_{i}}=n^{O(1/\lg\lg n)}$.
Therefore, $\beta_{i}=2^{O((\log^{7/8}n)(\log\log\log n))}\cdot n^{O(1/\lg\lg n)}=\Ohat(1)$.
\end{proof}
As the path-reporting $\Apxball^{\pi}$will call the distance-only
$\Apxball$ as a black-box, we will need the following bound.
\begin{prop}
\label{prop:ball time helper}For any $d'\le nW$ and $\eps'$ where
$\eps'\ge\eps_{0,\sigma_{\max}}$, we have $T_{\Apxball}(G,S,d',\eps')=\Otil(\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}})$.
\end{prop}

\begin{proof}
This follows from \Cref{thm:main no distance} when we set the accuracy
parameter $\eps'\gets\eps_{0,\sigma_{\max}}$ (we use $\eps'$ instead
of $\eps$ to avoid confusion). Note that $\eps_{0,\sigma_{\max}}\ge\phicmg^{2}$
satisfying \Cref{thm:main no distance}. In the proof of \Cref{thm:main no distance},
there are parameters $\eps'_{\distScale}=\eps'=\eps_{0,\sigma_{\max}}$
and $\eps'_{0}=\eps'/50^{\distScale}=\eps_{0,\sigma_{\max}}/50^{\distScale}$.
From \Cref{enu:induction ball} when $i=\distScale$, as $d'\le nW\le d'_{\distScale}$,
we have $T_{\Apxball}(G,S,d',\eps'_{\distScale})\le\Otil(\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}}{\phicmg(\eps'_{0})^{2}})=\Otil(\left|\ball_{G}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps{}_{0,\sigma_{\max}}^{2}})$.
\end{proof}
Now, we are ready to state the key inductive lemma that combines everything
together.
\begin{lem}
\label{lem:main path induction}For every $0\le i\le\distScale$ and
$0\le j\le\sigma_{\max}$, we can maintain the following data structures:
\begin{enumerate}
\item \label{enu:induction ball path}$\Apxball^{\pi}(G_{j},S,d',\eps_{i,j},\beta_{i})$
for any $d'\le d'_{i,j}\defeq32D_{i+1}\log(n)/\eps_{i,j}$ using total
update time of 
\[
\left|\ball_{G_{j}}(S,d')\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}2^{\distScale+\sigma_{\max}}}{\phicmg\eps_{0,\sigma_{\max}}}\right)=\Ohat(|\ball_{G_{j}}(S,d')|)
\]
with query-time overhead at most $(q_{\phi}^{(i,j)},q_{\path}^{(i,j)})$.
\item \label{enu:induction core path}$\Core^{\pi}(G_{j},\Kinit,d',\beta_{i})$
for any $d'\le D_{i+1}$ using total update time of 
\[
\left|\ball_{G_{j}}(\Kinit,32d'\log n)\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right)=\Ohat(|\ball_{G_{j}}(\Kinit,32d'\log n)|)
\]
with scattering parameter $\scatter=\Omega(\phicmg)$, stretch at
most $\stretch_{i}$, and query-time overhead at most $(Q_{\phi}^{(i,j)},Q_{\path}^{(i,j)})$.
\item $(D_{i},k_{i},\eps_{i,j},\stretch_{i},\Delta_{i},\beta_{i})$-covering
of $G_{j}$ using total update time of 
\[
\Otil(n\cdot\poly\left(\frac{n^{1/k_{0}+1/\distScale}2^{\distScale+\sigma_{\max}}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right))=\Ohat(n)
\]
 with query-time overhead at most $(Q_{\phi}^{(i,j)},Q_{\path}^{(i,j)})$.
\end{enumerate}
For all $i>0$, we assume by induction that a $(D_{i-1},k_{i-1},\eps_{i-1,j},\stretch_{i-1},\Delta_{i-1})$-covering
of $G_{j}$ is already explicitly maintained for every $0\le j\le\sigma_{\max}$.
\end{lem}

The rest of the section is for proving \Cref{lem:main path induction}.
Before proving \Cref{lem:main path induction}, we prove the main theorem
(\Cref{thm:main path}) using it. 

\paragraph{Proof of \Cref{thm:main path}.}

We apply \Cref{lem:main path induction} for $i=\distScale$ and $j=0$.
Recall that $G=G_{j}$, $\eps=\eps_{\distScale,0}$, $\beta_{\distScale}=\Ohat(1)$
by \Cref{prop:para path}(\ref{enu:para:beta}), $q_{\phi}^{(\distScale,0)}=c_{q}\sigma_{\max}\log n=O(\log^{2}n)$
and $q_{\path}^{(i,j)}=(2\distScale+1)\cdot\sigma_{\max}\cdot\overhead_{\path}=\Ohat(1)$.
Therefore, \Cref{lem:main path induction} gives us $\Apxball^{\pi}(G,S,d',\eps,\Ohat(1))$
data structure with $\Ohat(|\ball_{G}(S,d')|)=\Ohat(n)$ total update
time and $(O(\log^{2}n),\Ohat(1))$ query-time overhead as desired.

\subsection{Bounds for $\protect\Apxball^{\pi}$}

The proof is by induction on $i$ (starting from $0$ to $\distScale$)
and then on $j$ (starting from $\sigma_{\max}$ to $0$). We will
show that 
\[
T_{\Apxball^{\pi}}(G_{j},S,d',\eps_{i,j},\beta_{i})=(4^{i}2^{(\sigma_{\max}-j)})\cdot\left|\ball_{G_{j}}(S,d')\right|\cdot\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}
\]
for any $d'\le d'_{i,j}$ where $c'$ is some large enough constant,
which implies the claimed bound of $\left|\ball_{G_{j}}(S,d')\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}2^{\distScale+\sigma_{\max}}}{\phicmg\eps_{0,\sigma_{\max}}}\right)$. 

\paragraph{Base Cases ($i=0$).} For $i=0$ and any $j\in[0,\sigma_{\max}]$, the path-reporting ES-tree
from \Cref{prop:ES tree path} has total update time at most 
\begin{align*}
T_{\Apxball^{\pi}}(G_{j},S,d',\eps_{0,j},\beta_{0}) & \le O(\left|\ball_{G_{j}}(S,d')\right|d'\log n)\\
 & \le\left|\ball_{G_{j}}(S,d')\right|\cdot O(D_{1}\log^{2}(n)/\eps_{1})\\
 & \le\left|\ball_{G_{j}}(S,d')\right|\cdot(4^{i}2^{(\sigma_{\max}-j)})\cdot\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}.
\end{align*}
and query-time overhead of $(O(\log n),O(d'\log n))\le(q_{\phi}^{(i,j)},q_{\path}^{(i,j)}).$

\paragraph{The Inductive Step.} Below, we assume that $i>0$ and $j<\sigma_{\max}$. (The proof for
another base case when $j=\sigma_{\max}$ is exactly the same as below
but simpler, because we can ignore all terms related to $G_{j+1}$
as $G_{\sigma_{\max}+1}=\emptyset$.) We assume $d'>d'_{i-1,j}\defeq32D_{i}\log(n)/\eps_{i-1,j}$
otherwise we are done by induction hypothesis. 

\subparagraph{Total Update Time:}
\underline{Total Update Time:} As path-reporting $(D_{i-1},k_{i-1},\eps_{i-1,j},\stretch_{i-1},\Delta_{i-1},\beta_{i-1})$-covering
of $G_{j}$ is already explicitly maintained, we can implement $\Apxball^{\pi}(G_{j},S,d',\eps_{i,j},\beta_{i})$
where $\eps_{i,j}=300\eps_{i-1,j}+\eps_{i,j+1}$ and $\beta_{i}\ge8\Delta_{i-1}\beta_{i-1}$
via \Cref{thm:ball_path} using total update time of 
\begin{align*}
 & T_{\Apxball^{\pi}}(G_{j},S,d',\eps_{i,j},\beta_{i})\\
\le & \Otil(\left|\ball_{G_{j}}(S,d')\right|\Delta_{i-1}\frac{(32D_{i+1}\log(n)/\eps_{i,j})}{\eps_{i-1,j}D_{i-1}})+T_{\Apxball^{\pi}}(G_{j},S,2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1},\eps_{i-1,j},\beta_{i-1})+\\
 & T_{\Apxball^{\pi}}(G_{j+1},S,d',\eps_{i,j+1},\beta_{i})+T_{\Apxball}(G_{j+1},S,d',\eps_{i-1,j}).
\end{align*}
We will prove that $2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1},\eps_{i-1,j}\le d'_{i-1,j}$
so that we can apply induction hypothesis on $T_{\Apxball^{\pi}}(G_{j},S,2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1},\eps_{i-1,j},\beta_{i-1})$.
To see this, note that $D_{i}\ge\gamma_{i}D_{i-1}\ge(\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}})^{k_{i}}D_{i-1}$
by \Cref{prop:para path}(\ref{enu:para:gap and distance scale path}, \ref{enu:para:key path}). So 
\[
d'_{i-1,j}=\frac{32\log n}{\eps_{i-1,j}}D_{i}\ge\frac{32\log n}{\eps_{i-1,j}}\cdot(\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}})^{k_{i}}D_{i-1}\ge2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1}
\]
where the last inequality is because $k_{i}\ge k_{i-1}$ and $\frac{\stretch_{i}}{\eps_{i,\sigma_{\max}}}\ge\frac{\stretch_{i}}{\eps_{i,j}}\ge\frac{\stretch_{i-1}}{\eps_{i-1,j}}$
(because $\frac{\stretch_{i}}{\stretch_{i-1}}\ge600=\frac{\eps_{i,j}}{\eps_{i-1,j}}$).
Also, to apply induction hypothesis on $T_{\Apxball^{\pi}}(G_{j+1},S,d',\eps_{i,j+1},\beta_{i})$,
we note that $d'\le d'_{i,j}\le d'_{i,j+1}$ because $\eps_{i,j}\ge\eps_{i,j+1}$
by \Cref{prop:para path}(\ref{enu:para:eps path}). Therefore, the
bound on $T_{\Apxball^{\pi}}(G_{j},S,d',\eps_{i,j},\beta_{i})$ is
at most 

\begin{align*}
 & \Otil(\left|\ball_{G_{j}}(S,d')\right|\frac{n^{2/k_{i-1}+12/\distScale}}{\phicmg\eps_{i-1,j}^{2}})+T_{\Apxball^{\pi}}(G_{j},S,d'_{i-i,j},\eps_{i-1,j},\beta_{i-1})+\\
 & T_{\Apxball^{\pi}}(G_{j+1},S,d_{i,j+1},\eps_{i,j+1},\beta_{i})+T_{\Apxball}(G_{j+1},S,d',\eps_{i-1,j}).\\
\le & \left|\ball_{G_{j}}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}+(4^{i-1}2^{(\sigma_{\max}-j)})\cdot\left|\ball_{G_{j}}(S,d')\right|\cdot\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}\\
 & (4^{i}2^{(\sigma_{\max}-(j+1))})\cdot\left|\ball_{G_{j+1}}(S,d')\right|\cdot\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}+\left|\ball_{G_{j+1}}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}(\log n)^{c''}\\
\le & (2+2\cdot(4^{i-1}2^{(\sigma_{\max}-(j+1))}+4\cdot(4^{i-1}2^{(\sigma_{\max}-(j+1))})\times\left|\ball_{G_{j}}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}\\
\le & 4^{i}2^{(\sigma_{\max}-j)}\left|\ball_{G_{j}}(S,d')\right|\frac{n^{2/k_{0}+12/\distScale}50^{\distScale}}{\phicmg\eps_{0,\sigma_{\max}}^{2}}\cdot(\log n)^{c'}
\end{align*}
where the first inequality is by induction hypothesis and by \Cref{prop:ball time helper},
and the second inequality is because $G_{j+1}\subseteq G_{j}$ and
$c'\ge c''$ as $c'$ is chosen to be large enough. This completes
the inductive step for update time.

\underline{Query-time Overhead:} Since $2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1}\le d'_{i-1,j}$
and by induction hypothesis, we have $\Apxball^{\pi}(G_{j},S,2(\frac{\stretch_{i-1}}{\eps_{i-1,j}})^{k_{i-1}}D_{i-1},\eps_{i-1,j},\beta_{i-1})$
has query-time overhead at most $(q_{\phi}^{(i-1,j)},q_{\path}^{(i-1,j)})\le(Q_{\phi}^{(i-1,j)},Q_{\path}^{(i-1,j)})$.
Also, the path-reporting $(D_{i-1},k_{i-1},\eps_{i-1,j},\stretch_{i-1},\Delta_{i-1},\beta_{i-1})$-covering
of $G_{j}$ has query-time overhead at most $(Q_{\phi}^{(i-1,j)},Q_{\path}^{(i-1,j)})$
by induction hypothesis. Lastly, the query-time overhead of $\Apxball^{\pi}(G_{j+1},S,d',\eps_{i,j+1},\beta_{i})$
is at most $(q_{\phi}^{(i,j+1)},q_{\path}^{(i,j+1)})$ because $d'\le d'_{i,j}\le d'_{i,j+1}$.
Therefore, by \Cref{thm:ball_path}, the query-time overhead of $\Apxball^{\pi}(G_{j},S,d',\eps_{i,j},\beta_{i})$
is at most
\[
(q_{\phi}^{(i,j+1)}+O(1),\max\{q_{\path}^{(i,j+1)}+O(1),Q_{\path}^{(i-1,j)}+O(\frac{d'}{\eps_{i,j}D_{i-1}})\cdot Q_{\phi}^{(i-1,j)}\})\le(q_{\phi}^{(i,j)},q_{\path}^{(i,j)}).
\]
To see why the inequalities hold, we assume that $c_{q}$ is a large
enough constant. So, we have

\[
q_{\phi}^{(i,j+1)}+O(1)\le c_{q}(\sigma_{\max}-j)\log n+c_{q}\le q_{\phi}^{(i,j)}.
\]
Also, 
\[
q_{\path}^{(i,j+1)}+O(1)\le(2i+1)\cdot(\sigma_{\max}-j)\cdot\overhead_{\path}+c_{q}\le(2i+1)\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}=q_{\path}^{(i,j)}.
\]
Finally, 
\begin{align*}
Q_{\path}^{(i-1,j)}+O(\frac{d'}{\eps_{i,j}D_{i-1}})\cdot Q_{\phi}^{(i-1,j)} & \le2i\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}+\Otil(\frac{n^{2/k_{0}}}{\eps_{0,\sigma_{\max}}^{2}})\cdot(c_{q}\sigma_{\max}12^{\distScale}\log n)\\
 & \le2i\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}+\overhead_{\path}\\
 & =(2i+1)\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}=q_{\path}^{(i,j)}
\end{align*}
where $\overhead_{\path}=\frac{n^{2/k_{0}}\lenapsp}{\eps_{0,\sigma_{\max}}^{2}\phicmg^{2}}\log^{c_{q}}(n)\cdot\sigma_{\max}12^{\distScale}$.

\subsection{Bounds for $\protect\Core^{\pi}$}

The proof is by induction on $i$ (starting from $0$ to $\distScale$)
and we can fix any $j$.

\paragraph{Base Cases ($i=0$).} For $i=0$ and any $j\in[0,\sigma_{\max}]$, we have that a path-reporting
$(1,1,O(1),1)$-compressed graph of $G_{j}$ can be trivially maintained
by \Cref{prop:compressed base path}. By \Cref{thm:Core_path} and since
$\beta_{0}\ge7\lenapsp$ (by definition of $\beta_{0}$), we can implement
$\Core^{\pi}(G_{j},\Kinit,d',\beta_{i})$ with scattering parameter
$\scatter=\Omegatil(\phicmg)$ and stretch at most $\Otil(\gamma\lenapsp/\phicmg^{2})\le\stretch_{0}$
(by definition of $\stretch_{0}$) with total update time 
\begin{align*}
 & \Otil\left(T_{\Apxball^{\pi}}(G_{j},\Kinit,32d'\log n,0.1,\beta_{0})(D_{1})^{3}\lenapsp/\phicmg\right)\\
 & =\left|\ball_{G_{j}}(\Kinit,32d'\log n)\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right)
\end{align*}
by the ES-tree from \Cref{prop:ES tree path}. As the query-time overhead
of the $(1,1,O(1),1)$-compressed graph is $(1,1)$ by \Cref{prop:compressed base path}
and, by \Cref{prop:ES tree path}, the query-time overhead of $\Apxball^{\pi}(G_{j},S,4d',0.1,\beta_{i})$
is at most $(O(\log n),O(d'\log n))$. The query-time overhead of \\
$\Core^{\pi}(G_{j},\Kinit,d',\beta_{i})$ is at most $(O(\log n),\Otil(n^{1/k_{0}}\lenapsp/\phicmg^{2}))\le(Q_{\phi}^{(i,j)},Q_{\path}^{(i,j)})$.

\paragraph{The Inductive Step.}

\underline{Total Update Time:} For $i>0$ and and any $j\in[0,\sigma_{\max}]$, given that a path-reporting
$(D_{i-1},k_{i-1},\eps_{i-1,j},\stretch_{i-1},\Delta_{i-1},\beta_{i-1})$-covering
of $G_{j}$ is explicitly maintained, by \Cref{prop:covering-compressed is compressed path},
we can automatically maintain a $(D_{i-1},\gamma_{i-1},\Delta_{i-1},3\beta_{i-1})$-compressed
graph where $\gamma_{i-1}\ge(\stretch_{i-1}/\eps_{i-1,j})^{k_{i-1}}$
by \Cref{prop:para}(\ref{enu:para:key}) and because $\eps_{0,\sigma_{\max}}\le\eps_{i-1,j}$. By \Cref{thm:Core_path} and since $\beta_{i}\ge7\lenapsp\Delta_{i-1}\cdot(3\beta_{i-1})$,
we can maintain $\Core^{\pi}(G_{j},\Kinit,d',\beta_{i})$ with $\scatter=\Omegatil(\phicmg)$
and $\Otil(\gamma_{i-1}\lenapsp/\phicmg^{2})\le\stretch_{i}$ (by
definition of $\stretch_{i}$) with total update time 
\begin{align*}
 & \Otil\left(T_{\Apxball^{\pi}}(G_{j},\Kinit,32d'\log n,0.1)\Delta_{i-1}^{2}(D_{i+1}/D_{i-1})^{3}\lenapsp/\phicmg\right)\\
 & =\left|\ball_{G_{j}}(\Kinit,32d'\log n)\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right)
\end{align*}
by \Cref{enu:induction ball path} of \Cref{lem:main path induction}.

\underline{Query-time Overhead:} By \Cref{enu:induction ball path} of \Cref{lem:main path induction},
the query-time overhead of $\Apxball^{\pi}(G_{j},S,4d',0.1,\beta_{i})$
is at most $(q_{\phi}^{(i,j)},q_{\path}^{(i,j)})$. By induction hypothesis,
the path-reporting $(D_{i-1},k_{i-1},\eps_{i-1,j},\stretch_{i-1},\Delta_{i-1},\beta_{i-1})$-covering
has query-time overhead of $(Q_{\phi}^{(i-1,j)},Q_{\path}^{(i-1,j)})$
and so the query-time overhead of the $(D_{i-1},\gamma_{i-1},\Delta_{i-1},3\beta_{i-1})$-compressed
graph is at most $(3Q_{\phi}^{(i-1,j)},Q_{\path}^{(i-1,j)}+2Q_{\phi}^{(i-1,j)})$
by \Cref{prop:covering-compressed is compressed path}. Let $Q'_{\phi}=\max\{q_{\phi}^{(i,j)},3Q_{\phi}^{(i-1,j)}\}$
and $Q'_{\path}=\max\{q_{\path}^{(i,j)},Q_{\path}^{(i-1,j)}+2Q_{\phi}^{(i-1,j)}\}$.
By \Cref{thm:Core_path}, we have that the query-time overhead of $\Core^{\pi}(G_{j},\Kinit,d',\beta_{i})$
is at most 
\[
(4Q'_{\phi},Q'_{\path}+\Otil(\frac{d'}{D_{i-1}}\lenapsp/\phicmg^{2})\cdot Q'_{\phi})\le(Q_{\phi}^{(i,j)},Q_{\path}^{(i,j)}).
\]
To see why the inequalities holds, we first note that $Q'_{\phi}=3Q_{\phi}^{(i-1,j)}$
because $q_{\phi}^{(i,j)}=c_{q}(\sigma_{\max}-j+1)\log n\le c_{q}(\sigma_{\max}-j+1)12^{i-1}\log n=Q_{\phi}^{(i-1,j)}$.
So, we have
\[
4Q'_{\phi}=4\cdot\max\{q_{\phi}^{(i,j)},3Q_{\phi}^{(i-1,j)}\}=4\cdot3Q_{\phi}^{(i-1,j)}=Q_{\phi}^{(i,j)}.
\]
Also, we have
\begin{align*}
 & Q'_{\path}+\Otil(\frac{d'}{D_{i-1}}\lenapsp/\phicmg^{2})\cdot Q'_{\phi}\\
 & \le\max\{q_{\path}^{(i,j)},Q_{\path}^{(i-1,j)}+2Q_{\phi}^{(i-1,j)}\}+\Otil(\frac{n^{2/k_{0}}\lenapsp}{\phicmg^{2}})\cdot3Q_{\phi}^{(i-1,j)}\\
 & \le\max\{q_{\path}^{(i,j)}+\overhead_{\path},Q_{\path}^{(i-1,j)}+\overhead_{\path}\}\\
 & \le2(i+1)\cdot(\sigma_{\max}-j+1)\cdot\overhead_{\path}=Q_{\path}^{(i,j)}
\end{align*}
where $\overhead_{\path}=\frac{n^{2/k_{0}}\lenapsp}{\eps_{0,\sigma_{\max}}^{2}\phicmg^{2}}\log^{c_{q}}(n)\cdot\sigma_{\max}12^{\distScale}$.

\subsection{Bounds for Path-reporting Covering}

Recall that the algorithm from \Cref{thm:covering path} for maintaining
a path-reporting $(D_{i},k_{i},\eps_{i,j},\stretch_{i},\Delta_{i},\beta_{i})$-covering
of $G_{j}$ assumes, for all $D_{i}\le d'\le D_{i}(\frac{\stretch_{i}}{\eps_{i,j}})^{k}$,
$\Core^{\pi}$ and $\Apxball^{\pi}$ data structures with input distance
parameter $d'$. By \Cref{enu:induction ball path} and \Cref{enu:induction core path}
of \Cref{lem:main path induction}, we can indeed implement these data
structures for any distance parameter $d'\le D_{i+1}$. Since $D_{i}(\frac{\stretch_{i}}{\eps_{i,j}})^{k_{i}}\le D_{i}\gamma_{i}\le D_{i+1}$
by \Cref{prop:para}(\ref{enu:para:gap and distance scale},\ref{enu:para:key}),
the assumption is indeed satisfied by \Cref{enu:induction ball path}
and \Cref{enu:induction core path} of \Cref{lem:main path induction}.

So, using \Cref{thm:covering path}, we can maintain a path-reporting
$(D_{i},k_{i},\eps_{i,j},\stretch_{i},\Delta_{i},\beta_{i})$-covering
of $G_{j}$ with $\Delta_{i}=\Theta(k_{i}n^{2/k_{i}}/\scatter)$ in
total update time of 
\begin{align*}
O(k_{i}n^{1+2/k_{i}}\log n/\scatter+\sum_{C\in\cC^{ALL}}T_{\Core^{\pi}}(\stage G{t_{C}}_{j},\stage C{t_{C}},d_{\Clevel(C)},\beta_{i})\\
+T_{\Apxball^{\pi}}(\stage G{t_{C}}_{j},\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i,j}}32d_{\Clevel(C)},\eps_{i,j},\beta_{i}))
\end{align*}
where $\cC^{ALL}$ contains all cores that have ever been initialized
and, for each $C\in\cC^{ALL}$, $t_{C}$ is the time $C$ is initialized.
By plugging in the total update time of $\Apxball^{\pi}$ from \Cref{enu:induction ball path}
and $\Core^{\pi}$ from \Cref{enu:induction core path}, the total
update time for maintaining the covering is 
\begin{align*}
\Otil(\frac{n^{1+2/k_{i}}}{\scatter}+\sum_{C\in\cC^{ALL}}\left|\ball_{\stage G{t_{C}}_{j}}(\stage C{t_{C}},32d_{\Clevel(C)}\log n)\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right)+\\
\left|\ball_{\stage G{t_{C}}_{j}}(\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i,j}}d_{\Clevel(C)})\right|\poly\left(\frac{n^{1/k_{0}+1/\distScale}2^{\distScale+\sigma_{\max}}}{\phicmg\eps_{0,\sigma_{\max}}}\right)).
\end{align*}
As it is guaranteed by \Cref{thm:covering path} that 
\[\sum_{C\in\cC^{ALL}}|\ball_{\stage G{t_{C}}_{j}}(\stage C{t_{C}},\frac{\stretch_{i}}{4\eps_{i,j}}d_{\Clevel(C)})|\le O(k_{i}n^{1+2/k_{i}}/\scatter),
\]
and therefore the above expression simplifies to $\Otil\left(n\cdot\poly\left(\frac{n^{1/k_{0}+1/\distScale}2^{\distScale+\sigma_{\max}}\lenapsp}{\phicmg\eps_{0,\sigma_{\max}}}\right)\right)$.
As the query-time overhead of all invoked instances of $\Core^{\pi}$
and $\Apxball^{\pi}$is at most $(Q_{\phi}^{(i,j},Q_{\path}^{(i,j)})$
by \Cref{enu:induction ball path} and \Cref{enu:induction core path}
of \Cref{lem:main path induction}, the query-time overhead of the
covering $\cC$ is at most $(Q_{\phi}^{(i,j},Q_{\path}^{(i,j)})$
by definition.

